On Evaluation of Document Classification using RVL-CDIP

The RVL-CDIP benchmark is widely used for measuring performance on the task of document classification. Despite its widespread use, we reveal several undesirable characteristics of the RVL-CDIP benchmark. These include (1) substantial amounts of label noise, which we estimate to be 8.1% (ranging between 1.6% to 16.9% per document category); (2) presence of many ambiguous or multi-label documents; (3) a large overlap between test and train splits, which can inflate model performance metrics; and (4) presence of sensitive personally-identifiable information like US Social Security numbers (SSNs). We argue that there is a risk in using RVL-CDIP for benchmarking document classifiers, as its limited scope, presence of errors (state-of-the-art models now achieve accuracy error rates that are within our estimated label error rate), and lack of diversity make it less than ideal for benchmarking. We further advocate for the creation of a new document classification benchmark, and provide recommendations for what characteristics such a resource should include.

==> rules.tex <==
\begin{table*}
\centering
\scalebox{0.72}{
    \begin{tabular}{l m{8cm} m{7cm}}
        \toprule
        \textbf{Category} & \textbf{Description} & \textbf{Notes and Observations}\\
        \midrule
        \texttt{advertisement} & Advertisements from print-form media like newspapers and magazines. Also a small amount of scripts for television or radio advertisements. A small amount of "ad order instructions" and "ad insertion" documents. & \\
        \midrule
        \texttt{budget} & Includes various budget documents such as expense, spending, sales, cash, and accounting reports and forecasts; budgets; quotes and estimates; and income and bank statements. Also includes receipt-like documents such as political campaign contribution requests and other receipts, as well as checks and check stubs.  & \\
        \midrule
        \texttt{email} & Scanned images of printed emails. & \\
        \midrule
        \texttt{file\_folder} & Scanned images of folders and binders. Folder scans are often characterized by vertically oriented text (indicating a folder label). & A moderate amount of file folders contain handwritten text or notes. Some scanned folders may be indistinguishable from blank pages.\\
        \midrule
        \texttt{form} & & \\
        \midrule
        \texttt{handwritten} & includes handwritten documents like handwritten letters and scientific notes & \\
        \midrule
        \texttt{invoice} & Includes invoices, bills, and account statements. & \\
        \midrule
        \texttt{letter} & Letters, often with letterhead and commonly with ``Dear..." salutations. & The distinction between letters and memos is often unclear. \\
        \midrule
        \texttt{memo} & Memoranda or inter-office correspondence documents, often with clear ``TO", ``FROM", ``SUBJECT" headings. & \\
        \midrule
        \texttt{news\_article} & Includes news articles in the form of clippings from newspapers and other print-form news media, as well as a small amount of news articles from the web. Also includes press releases.  & press releases -- might overlap with presentation\\
        \midrule
        \texttt{presentation} & Includes scanned images of presentation and overhead slides, transcripts of speeches and statements. Also includes a large amount of press releases. &  \\
        \midrule
        \texttt{questionnaire} & Includes customer surveys and questionnaires, as well as survey and questionnaire prompts for surveyors. Also includes questionnaires appearing to be part of legal proceedings and investigations. & Many questionnaires have a substantial amount of form-like elements.\\
        \midrule
        \texttt{resume} &
        Includes resumes, curricula vitae (CVs), biographical sketches, executive biographies (e.g., those written in third-person), a small amount of business cards. & contains a large amount of social security numbers and other personally-identifiable information like dates-of-birth and addresses \\
        \midrule
        \texttt{scientific\_pub.} & Mainly papers and articles from scientific journals and book chapters, but also includes book title pages. Also includes news articles from science newsletters. & News articles from science newsletters are very similar to the \texttt{news\_article} category.\\
        \midrule
        \texttt{scientific\_rep.} & Includes bioassay, pathology, and test reports; charts, graphs, and tables; research reports (including progress reports), research proposals, abstracts, paper drafts & Many reports and abstracts bear similarities to scientific publications. Many test results are similar to specifications.\\
        \midrule
        \texttt{specification} & Data sheets (including safety data sheets); product, material, and test specifications. Also includes specification change reports. & \\
        \bottomrule
    \end{tabular}}
    \caption{RVL-CDIP categories alongside our descriptions.}
    \label{tab:label-guidelines}
\end{table*}
